Deep Ranking with Adaptive Margin Triplet Loss

We propose a simple modification from a fixed margin triplet loss to an adaptive margin triplet loss. While the original triplet loss is used widely in classification problems such as face recognition, face re-identification and fine-grained similarity, our proposed loss is well suited for rating datasets in which the ratings are continuous values. In contrast to original triplet loss where we have to sample data carefully, in out method, we can generate triplets using the whole dataset, and the optimization can still converge without frequently running into a model collapsing issue. The adaptive margins only need to be computed once before the training, which is much less expensive than generating triplets after every epoch as in the fixed margin case. Besides substantially improved training stability (the proposed model never collapsed in our experiments compared to a couple of times that the training collapsed on existing triplet loss), we achieved slightly better performance than the original triplet loss on various rating datasets and network architectures.

==> unrelated_work.tex <==
\section{(Un)-Related Work}

Quoted from \cite{Wu_sampling_2017}: \enquote{Triplet loss is currently among the best-performing losses on standard embedding tasks.}

Cite papers about ranking

https://arxiv.org/pdf/1705.00105.pdf (for more citations)

https://devavrat.mit.edu/wp-content/uploads/2017/11/Iterative-ranking-from-pair-wise-comparisons.pdf

https://pdfs.semanticscholar.org/ea65/c0cd0ccbd432f8a9c96a61caa62ce48f4a0b.pdf

https://dl.acm.org/citation.cfm?id=2063675

https://medium.com/@akarshzingade/image-similarity-using-deep-ranking-c1bd83855978

OASIS: http://www.jmlr.org/papers/volume11/chechik10a/chechik10a.pdf
